Camera Alignment and Weighted Contrastive Learning for Domain Adaptation in Video Person ReID

Systems for person re-identification (ReID) can achieve a high accuracy when trained on large fully-labeled image datasets. However, the domain shift typically associated with diverse operational capture conditions (e.g., camera viewpoints and lighting) may translate to a significant decline in performance. This paper focuses on unsupervised domain adaptation (UDA) for video-based ReID - a relevant scenario that is less explored in the literature. In this scenario, the ReID model must adapt to a complex target domain defined by a network of diverse video cameras based on tracklet information. State-of-art methods cluster unlabeled target data, yet domain shifts across target cameras (sub-domains) can lead to poor initialization of clustering methods that propagates noise across epochs, thus preventing the ReID model to accurately associate samples of same identity. In this paper, an UDA method is introduced for video person ReID that leverages knowledge on video tracklets, and on the distribution of frames captured over target cameras to improve the performance of CNN backbones trained using pseudo-labels. Our method relies on an adversarial approach, where a camera-discriminator network is introduced to extract discriminant camera-independent representations, facilitating the subsequent clustering. In addition, a weighted contrastive loss is proposed to leverage the confidence of clusters, and mitigate the risk of incorrect identity associations. Experimental results obtained on three challenging video-based person ReID datasets - PRID2011, iLIDS-VID, and MARS - indicate that our proposed method can outperform related state-of-the-art methods. Our code is available at: \url{https://github.com/dmekhazni/CAWCL-ReID}

==> Backup/Methodology_old.tex <==
 In this section, the overall approach shown in Figure \ref{fig:overall_framewotk} is presented module by module.
Most methods for Video ReID learn to associate tracklets to the correct identity through a clustering approach based on pseudo-labels.  
However, those method strongly rely on the quality of the pseudo-labels in the early training iterations. Poor initialization will prevent iterative convergence and the whole training process will fail. We propose a novel training process based on domain adaptation that starts by consolidating the performances of the encoder on the Target dataset with an Adversarial Camera confusion technique. After improving the cluster quality thanks to previous step, the network can start the self-paced pseudo-label based training. Self-paced is essential to estimate bad clusters and avoid encouraging wrong directions during the training. From our best knowledge, we are the first using the camera ID information to decrease the encoder discrimination on the Target set.
    
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/overall_archi.PNG}
    \caption{Video-based UDA ReID overall framework. Source and taget tracklets are processed by the backbone $\mathcal{M}$ and a representation $g(Tk)$ is computed. The training loss $\mathcal{L}$ is composed of three part: the supervised cross-entropy loss on the source tracklets ($\mathcal{L}_{CE}$), camera confusion loss on source and target tracklets ($\mathcal{L}_{Cam}$) and cotrastive loss ($\mathcal{L}_{Contr}$), which uses a memory bank of clustered and unclustered tracklets. }
    \label{fig:overall_framewotk}
\end{figure*}


%%%%%%%%
\subsection{Tracklet Representation}

    Given a set $\data$ of $N$ tracklets, each tracklet is composed of a sequence of $N_\trk$ images $\{x_1, \ldots, x_{|N_\trk|}\}$. We consider that the first $N_s < N$ tracklets are from a source domain $S$ and come with a personID label $y$, while the remaining $N_t = N-N_s$ ones are from a target domain for which there is no person ID. The goal is to learn a function $f$ mapping images $x$ to a representation vector $f(x)$ which is able to discriminate identities, i.e. find separable distances to consider two pairs as same individual or no, while being robust to differences between the source and target domains. 
    
    Since input data are tracklets, a features aggregator is employed so that each video-sequence has its own unique representation.  The aggregation method TCLNet proposed by Hou \cite{hou2020temporal} is adopted. By exploiting spatio-temporal information, TCLNet is the association of two modules, Temporal Saliency Erasing (TSE) and Temporal Saliency Boosting (TSB). 
    We denote the representation of a tracklet through the backbone $\mathcal{M}$ as $g(\trk)$.
    %The representation of a tracklet $\trk$ is given by {$g(\trk)$} = TCLNet($\trk$).
    \newline
    \textbf{Clips:} In the video-based context, it happens that tracklets contain different mode. Between the starting frame and the final frame, events could have arrived (occlusion, change in trajectory, ...). From this observation, we proposed to split each tracklet $\trk$ into $N_\Omega$ equal-sized clips $\Omega$. The tracklet becomes then $\trk = \{\Omega_0, ..., \Omega_{Nc} \}$

%%%%%%%%
\subsection{Training Strategy}
    An association of a supervised loss, a camera confusion loss and a self-paced contrastive learning loss for domain adaptation is proposed as follow:    
        \begin{equation}
        \loss \, = \, \delta_1\lossSup \, \, + \, \delta_2\lossCam \, + \delta_3\lossContr.
        \end{equation}
    where $\lossSup$ refers to the supervised training on source = S domain, $\lossCam$ refers to the camera classifier to avoid learning camera-identity related, and $\lossContr$ refers to the contrastive loss on clustered samples.    
 
    \mypar{1) Supervised Loss:}  The first loss, which uses only source data, ensures that the tracklet representation $g(\trk)$ can be used for identity classification through an identity classifier $\theta_I$. It converts $g(\trk)$ to a class probability vector with a linear layer followed by a softmax, and uses cross-entropy as classification loss. It can be expressed as:
        %\begin{equation}
            %\lossSup \ = \ - \frac{1}{N_s} \sum_{i=1}^{N_s} \sum_{k=1}^K \, \log \frac{\exp\big(\tr{c}_k g(\trk_i)\big)}{\sum_{l} \exp\big(\tr{c}_l g(\trk_i)\big)},
            %\label{eq:LossSup}
        %\end{equation}
%where $c_k$ is the weight vector corresponding to class $k \in \{1,\ldots,K\}$.
    \begin{equation}
        \mathcal{L}^{\mr{\textsc{ce}}} =
        \frac{1}{K}\sum_i^K
        -\log \left( \frac{ \exp ( {W^T_{y_i} g(\trk_i) + b_{y_i}} ) } {\sum_{j=1}^{N_I} \exp{ ( W_{j}^T g(\trk_i) + b_j} ) }   \right)
    \end{equation}
    where $K$ is the batch size.  Class label $y_{i} \in \{1, 2, ..., N_I\}$ is associated with training tracklet g($\trk_i$), the $i^{th}$ training tracklet. Weight vectors $W_{yi}$ and bias $b_{yi}$ of last fully connected (FC) layer corresponds to class $y$ of $i^{th}$ tracklet. $W_{j}$ and $b_{j}$  are weights and bias of last FC corresponding of the $j^{th}$ class ($j \in [1, N_I]$). $W_j$ and $W_{y_i}$ are respectively the $j^{th}$ and $y_i^{th}$ column of $W = \{ w_{ij} : i = 1, 2, ..., F; j = 1, 2, ..., N_I\}$, where $F$ is the size of the last FC layer of the backbone.
    
    \mypar{2) Camera-Level Confusion:} \label{clc}  We empirically observed a miss-alignment of target = T inter camera distributions after the pre-training on the Source dataset. This lack of alignment yield poor initial pseudo-labels.  Inspired by \cite{ganin2015unsupervised} we use an adversarial distribution alignment approach. We propose to align the per-camera distribution rather than the domains. A camera classifier $\theta_c$ is trained to discriminate the target = T cameras with a cross entropy loss, the gradient of this loss is inverted with a Gradient Reversal Layer (GRL) and back-propagated through the encoder. This reversed objective aims to remove the information related to the camera scene from the representation and helps to make the source and target domains indistinguishable for the classifier. Using the cross-entropy loss to train the camera classifier incentives the encoder to minimize the classifier accuracy, which can be unstable.
    
    \begin{equation}
        S_i =         
         \left( \frac{ \exp ( {W^T_{c_i} \theta_c(g(\trk_i)) } ) } {\sum_{j=1}^{N_c} \exp{ ( W_{j}^T \theta_c(g(\trk_i)) } ) }   \right)
        \label{eq:Si_camcla}
    \end{equation}    
    \begin{equation}
        \loss^{\mr{\textsc{ce}}}_{\mr{cam}}     
        \frac{1}{K}\sum_i^K
        -\log \left( \frac{ \exp ( {W^T_{c_i} \theta_c(g(\trk_i)) } ) } {\sum_{j=1}^{N_c} \exp{ ( W_{j}^T \theta_c(g(\trk_i)) } ) }   \right)
        \label{eq:CE_camcla}
    \end{equation}
    where $N_c$ is the number of cameras $T$ in the target domain.  We therefore propose a novel confusion loss to train the camera classifier, defined as follows:
            \begin{equation}
            \begin{aligned}
         \loss^{\mr{\textsc{guce}}}_{\mr{cam}} =  & \quad
        \frac{1}{N_b^2} \left[\sum^{N_b}_{i=1}\log \frac{\exp c_{y_i,i}}{\sum_{j=1}^{N_c}\exp(c_{j,i})}\right].
        \\
        & \quad
        \left[\sum^{N_b}_{i=1}\log \frac{\exp (    
        1 -
        c_{y_i,i})}{\sum_{j=1}^{N_C}\exp( 1- c_{j,i})}\right]
         \end{aligned}
        \end{equation}
        where $c_{j,i}$ is the output of the classifier for camera $j$ and sample $i$.        
            %\begin{equation}
                %\lossCam^{GUCE} = %\lossSup(LS(D(f(x)),y) \cdot %\lossSup(LS(1-S(D(f(x))),y)
                %\label{eq:confusion_loss}
            %\end{equation}
    %where $LS$ and $S$ are respectively the log softmax and softmax function, and $D$ is the camera classifier.     
    This loss, encourages the classifier to be sure about his predictions, may they be right or wrong. The encoder is then encouraged to maximise the classifier confusion, i.e maximise the conditional entropy $H(C|g(\trk))$ where $C$ is the distribution of cameras and the distribution of tracklets. A similar confusion based loss for adversarial approaches was proposed in \cite{InformationTheoricReg}.
    
    % \subsubsection{Camera-level confusion}
    %     Contrary to the original paper, that uses this techniques to shorten the domain gap between the Source and the Target datasets, this work rely on another architectural granularity, with a camera classifier rather than a domain classifier. This allows to align the representations of the Target cameras together, as we empirically observed that pre-training on the source was not sufficient for the inter-camera representations of the Target Identities to be aligned. Our method therefore explicitly remove the camera-specific information from the Target representation. Finally, we extended the method to also align the Source and Target datasets, as done in the original paper, by adding the Source camera to the same classifier head, and summing over the probabilities of each domain cameras to obtain the probability of each domain. The resulting domain and camera confusion loss is :
        % \begin{equation}
        %         \loss_{GDC} = \loss_{DBC} + \loss_{CBC} 
        % \end{equation}

        % To this day we haven't explored the possibility of balancing the domain and camera BC loss.

    \mypar{3) Contrastive Loss} The contrastive loss is based on positives and negatives pairs of tracklets on Source and pseudo-positive/negatives pairs, i.e. pairs of samples assimilated to same cluster or not, on target and is defined as follow:
            \begin{equation}\label{eq:lossContr}
                \lossContr \ = \ \frac{1}{N} \sum_{i=1}^N \sum_{j\neq i} \log \frac{\exp\left(\tr{\normg(\trk_i)} \normg(\trk_j)\right)}
                {\sum\limits_{j' \neq i} \exp\left(\tr{\normg(\trk_i)} \normg(\trk_{j
                '})\right)} 
            \end{equation}
    where $\normg(\trk) = g(\trk) \mathbin{/} \|g(\trk)\|$.
%$\normg(\trk) = \frac{g(\trk)}{\|g(\trk)\|}$.
This loss helps to adapt the tracklets representations such that different identities can be easily distinguished on both source and target data.
%%%%%%%%%%%%%%%%%%%%%
\subsection{Association of Pseudo-Labels}

    %In this section, two approaches are presented to generate pseudo-labels. One rely on an existing clustering algorithm \cite{SPCL},  and the other based on observations of distances. As batch size is restricted for machine resources, a memory bank \cite{MoCoHe} is used to contrast on the whole training set.
    Im this section we present the technique that we use to associate psuedo-labels to the target tracklets (for which we do not have real labels) to be used for the contrastive loss.
    As the tracklets memory footprint is large, a memory bank \cite{MoCoHe} is used to contrast on the whole training set.
    Finally, we introduce a self-paced strategy to further improve the quality of the pseudo-labels.
    
    \mypar{1) Generation of Pseudo-Labels:} To generate pseudo-labels, DBSCAN clustering algorithm is used. A Jaccard distance matrix, calculated based on the $k$-reciprocal nearest neighbours sets, is used for this clustering phase. The choice of such a metric enforce more robust clusters. Indeed, samples that share reciprocal neighbors tend to form positive pairs \cite{SPCL, RerankingZhong}.
    
    
    % on similarity matrix produced with Jaccard distances. The Jaccard distance allow to take in consideration not only ...
    % Assume that the distance between two samples $x_1$ and $x_2$ is measured using $d(x_1, x_2) = (x_1 - x_2)^T(x_1 - x_2)$. For a given sample $p$ in the training set, a $k$-Nearest Neighbour ($k$NN) computed the distance with all other samples in the training set for the target $X^t$ domain:
    %         \begin{equation}
    %             N(p,X^t) = \{x_1^t, x_2^t, ..., x_n^t\},  \ |N(p, k)| = k
    %         \end{equation}
    % Assuming that two samples from the same identity should be reciprocally in the other $k$NN set, the $k$-reciprocal nearest neighbours set $R$ can be defined as:
    %         \begin{equation}
    %             R(p,k) = \{x_i | (x_i \in N(p, k)) \And (p \in N(x_i, k)) \}
    %         \label{rknn}
    %         \end{equation}
    %         The Jaccard distance $d_J$ can now recalculate distance between two sample but based on their reciprocal k-NN set so that it measure the overlap in each respective k-NN set.
    %         \begin{equation}
    %             d_J(p, x_i) = 1 - \frac
    %             {|R(p, k) \bigcap R(x_i, k)|}
    %             {|R(p, k) \bigcup R(x_i, k)|}
    %         \end{equation}
    %         DBSCAN is then applied on the matrix similarity filled with all distances between samples in the train set to generate clusters.
            
            \begin{figure}
                \centering
                \begin{subfigure}{0.4\textwidth}
                    \includegraphics[width=\textwidth]{Figures/camera_confusion.png}
                    \caption{}
                    \label{fig:camera_confusion}
                \end{subfigure}
                \hfill
                \begin{subfigure}{0.45\textwidth}
                    \includegraphics[width=\textwidth]{Figures/knn_weighting.PNG}
                    \caption{}
                    \label{fig:weight_criterion}
                \end{subfigure}
                \caption{Figure \ref{fig:camera_confusion} presents a scenario before and after camera alignment. Figure \ref{fig:weight_criterion} present our Weighting strategies to define gamma. Left is kNN based gamma estimation ($k$=4 in this example).}
            \label{fig:figures}
            \end{figure}
    
    
    \mypar{2) Self-Paced Strategy:} Let $w_{ij} \in [0,1]$ be a self-paced weight representing the likeliness that tracklets $\trk_i$ and $\trk_j$ correspond to the same person. For labeled source examples, we set $w_{ij}=1$ if $y_i = y_j$, and otherwise $w_{ij}=0$. 
            
    In the case of source examples, for which the weight $w_{ij}$ is known, the first term in the sum corresponds to the supervised contrastive loss of \cite{khosla2020supervised}. On the other hand, for target examples, we need to optimize both embedding function $f$ and self-paced weights $w_{ji}$. The update of self-paced weights is controlled by a self-paced regularization function $R_\gamma$, parameterized by the learning pace $\gamma > 0$. This function has the property of being monotone decreasing with respect to the loss (i.e., harder examples are given less importance) and monotone increasing with respect to the learning (i.e., a larger $\gamma$ increases the weights). 
    Here, we consider for this function a linear self-paced learning:    
        \begin{equation}
            R_\gamma(w_{ij}) = -\gamma w_{ij}.
        \end{equation}       
    %Here, we consider two popular choices for this function based on hard and linear self-paced learning:    
        %\begin{align}
            %R_\gamma^{\mr{hard}}(w_{ij}) & = -\gamma w_{ij}  \\
            %\quad R_\gamma^{\mr{linear}}(w_{ij}) & = \gamma %\big(\tfrac{1}{2}w^2_{ij} - w_{ij}\big).
        %\end{align}    
    The self-paced contrastive loss (\ref{eq:lossContr}) can then be written as
        \begin{equation}
            \lossContr \ = \ \frac{1}{N} \sum_{i=1}^N \sum_{j\neq i} w_{ij}  l_{ij} \, + \, R_\gamma\big(w_{ij}\big)
        \end{equation}
    where    
        \begin{align}\label{eq:lij}
            l_{ij} 
            & =  - \log \frac{\exp\left(\tr{\normg(\trk_i)} \normg(\trk_j)\right)}
            {\sum\limits_{j' \neq i} \exp\left(\tr{\normg(\trk_i)} \normg(\trk_{j
            '})\right)}
            % \\
            % & = \ \log\,\sum_{j'\neq i} \exp\underbrace{\Big(\tr{\normg(\trk_i)}\big( \normg(\trk_{j'})-\normg(\trk_{j}\big)\Big)}_{\leq \, 2}
        \end{align}
    Since $l_{ij} \geq 0$ and $w_{ij} \in [0,1]$, the optimal weights can be obtained in closed-form for a fixed embedding function $f$ as:
        \begin{align}
            w_{ij} =  \max\Big(1-\frac{1}{\gamma}l_{ij}, \, 0\Big).
        \label{eq:sp-weights}
        \end{align}        
        %\begin{align}\label{eq:sp-weights}
        %    w_{ij}^{\mr{hard}} & \ = \ \left\{\begin{array}{ll}
        %    1, & \tx{ if } l_{ij} \leq \gamma\\
        %    0, & \tx{ else}
        %    \end{array}\right.\\
        %    w_{ij}^{\mr{linear}} & \ = \ %\max\Big(1-\frac{1}{\gamma}l_{ij}, \, 0\Big).
        %\end{align}            
    The overall optimization process is as follows. Starting with a small learning rate $\gamma_0 \approx 0$, at each iteration, we alternate between updating the embedding function $f$ and classifier parameter $c_k$ using gradient descent and updating the weights $w_{ij}$ as in (\ref{eq:sp-weights}). At the end of each iteration, the learning pace can be increased according to some fixed policy, for instance $\gamma := (1+\alpha)\gamma$, with $\alpha > 0$. In our method, we set $\gamma$ based on the maximum distance between an example and its $k$-nearest neighbor.
    
    %Note that, based on (\ref{eq:lij}) , we have that the following bounds on $l_{ij}$: $0 \leq l_{ij} \leq \log(N\!-\!1)+2$. Hence, $\gamma$ can be updated to range from $0$ to $\log(N\!-\!1)+2$ within a pre-determined number of iterations. %{\color{red}CD: Not sure about the $\log(N-1)$ part, need to verify it...}            
        
    \mypar{3) Memory bank:} To alleviate memory issues and allow the full use of all data for the contrastive loss, allowing a more reliable comparison pairs to pairs at each batch step, a memory bank is employed to store the features of all samples at the beginning of each epoch.
    Clustered samples have the mean of the features belonging to the same cluster $\Psi_i$, with i the i-th cluster, saved in the memory. For unclustered samples we save their features $g(\trk_j)$ directly, with j the j-th sample unclustered.
    It consist into considering a query q and a set of encoded samples \{$k_0, k_1, ...$ \} that are keys of a dictionary. The contrastive loss \ref{eq:lossContr} is then calculated considering samples in the batch as q and all other samples store in the dict as keys. The backpropagation and weight update for the encode are made only with samples in the batch, the keys being detached from the graph are not included. To avoid memory issues in storing all the graph for them due to memory issues, we update the keys differently, according to the following rule:
            \begin{equation}
                \theta_k \leftarrow m\theta_k + (1 - m)\theta_q.
            \end{equation}
    In this context, $m \in [0, 1]$ and $\theta_k$ (resp. $\theta_q)$ refers to the representation of the keys (resp. query).

==> Chapters/SuppMaterial.tex <==
\subsection{Visualizations}

    In this section, activation map visualizations are represented. Figure \ref{fig:actmap} represents the better localization for the features across the proposed method. Compared to the baseline SPCL, less background information is captured and allow the model to focus properly on strong identity-based features.

    \begin{figure*}[!ht]
         \centering
         \includegraphics[width=0.9\textwidth]{Figures/Supplementary/actmap.png}
         \caption{Three individuals from the target represented. Top is from the baseline SPCL and bottom is our proposed approach. The first image represent the sample, the middle is the activation map and the last image is the superposition of the sample with the activation map.}
        \label{fig:actmap}
    \end{figure*}
     
\subsection{Impact of the number of frames per Tracklets}

    This section deals with the number of frames per tracklet. We can observe Table \ref{tab:frames_per_tracklet} that since we cut each tracklet in equal chunks to maintain scalability to all the dataset, the temporal information remains stable from 4 frames per tracklets and so performances does not differ much. In this context, we assume that keeping the number of frames per tracklets to the minimal acceptable value (4 in our case) is suitable for high memory consumption task (i.e. video-based ReID).
    
    \begin{table}[!ht]
        \begin{tabular}{|c|cc|cc|cc|}
            \hline
            \multirow{Number of frames per tracklet} & \multicolumn{2}{c|}{PRID2011}      & \multicolumn{2}{c|}{iLIDS-VID}     & \multicolumn{2}{c|}{MARS}          \\ \cline{2-7} 
                                                           & \multicolumn{1}{c|}{mAP}  & Rank-1 & \multicolumn{1}{c|}{mAP}  & Rank-1 & \multicolumn{1}{c|}{mAP}  & Rank-1 \\ \hline
            2                                              & \multicolumn{1}{c|}{89.2} & 91.6   & \multicolumn{1}{c|}{74.5} & 80.4   & \multicolumn{1}{c|}{83.8} & 77.0   \\ \hline
            4                                              & \multicolumn{1}{c|}{92.1} & 94.5   & \multicolumn{1}{c|}{76.0} & 84.0   & \multicolumn{1}{c|}{86.9} & 81.8   \\ \hline
            8                                              & \multicolumn{1}{c|}{91.9} & 94.2   & \multicolumn{1}{c|}{76.2} & 84.0   & \multicolumn{1}{c|}{86.6} & 80.6   \\ \hline
            16                                             & \multicolumn{1}{c|}{92.0} & 94.9   & \multicolumn{1}{c|}{75.7} & 84.2   & \multicolumn{1}{c|}{87.1} & 81.3   \\ \hline
        \end{tabular}
        \label{tab:frames_per_tracklet}
        \caption{Results for a supervised training using different frames per tracklets. }
    \end{table}
